Efficient Finetuning for Dimensional Speech Emotion Recognition in the Age of Transformers

Accurate speech emotion recognition is essential for developing human-facing systems. Recent advancements have included finetuning large, pretrained transformer models like Wav2Vec 2.0. However, the finetuning process requires substantial computational resources, including high-memory GPUs and significant processing time. As the demand for accurate emotion recognition continues to grow, efficient finetuning approaches are needed to reduce the computational burden. Our study focuses on dimensional emotion recognition, predicting attributes such as activation (calm to excited) and valence (negative to positive). We present various finetuning techniques, including full finetuning, partial finetuning of transformer layers, finetuning with mixed precision, partial finetuning with caching, and low-rank adaptation (LoRA) on the Wav2Vec 2.0 base model. We find that partial finetuning with mixed precision achieves performance comparable to full finetuning while increasing training speed by 67%. Caching intermediate representations further boosts efficiency, yielding an 88% speedup and a 71% reduction in learnable parameters. We recommend finetuning the final three transformer layers in mixed precision to balance performance and training efficiency, and adding intermediate representation caching for optimal speed with minimal performance trade-offs. These findings lower the barriers to finetuning speech emotion recognition systems, making accurate emotion recognition more accessible to a broader range of researchers and practitioners.

==> tables/shared_table.tex <==
\begin{table*}[h]
    \caption{Wav2Vec 2.0 training results on NVIDIA A40 (non-caching) and RTX 2080 Ti (caching). We report results for single precision (SP) and mixed precision (MP) separately. We report the number of transformer layers trained (`Layers'), activation and valence CCC on MSP-Podcast ``Test1" split (`Act' and `Val'), wall-clock training time in hours for 5 epochs in both caching (`Time C') and non-caching (`Time NC') setups, and number of trainable parameters for caching (`Params C') and non-caching (`Params NC').  * indicates statistically significant difference from full 12-layer finetune. Caching performance is not statistically different from its non-caching counterparts, except for 3-layer MP activation, where caching performs worse.}
    \label{tab:combined_results_table}
    \centering
    \begin{tabular}{l c c c c c c c}
        \hline
        \textbf{Layers} & \textbf{Precision} & \textbf{Act} & \textbf{Val} & \textbf{Time NC (h)} & \textbf{Time C (h)} & \textbf{Params NC} & \textbf{Params C} \\
        \hline
        \multirow{1}{*}{LoRA} & SP & 0.623±0.02 & 0.506*±0.01 & 2.476±0.015 & -- & 300K & -- \\
        \hline
        \multirow{2}{*}{1} & SP & 0.622±0.02 & 0.458*±0.01 & 2.443±0.002 & 0.35±0.00 & \multirow{2}{*}{12M} & \multirow{2}{*}{7M} \\
                           & MP & 0.625±0.01 & 0.462*±0.01 & 0.965±0.01 & 0.16±0.01 \\
        \hline
        \multirow{2}{*}{2} & SP & 0.638±0.01 & 0.508*±0.01 & 2.477±0.013 & 0.69±0.00 & \multirow{2}{*}{19M} & \multirow{2}{*}{14M} \\
                           & MP & 0.645±0.01 & 0.507*±0.004 & 0.982±0.003 & 0.25±0.00 \\
        \hline
        \multirow{2}{*}{\textbf{3}} & SP & 0.648±0.01 & 0.565±0.002 & 2.519±0.017 & 1.02±0.00 & \multirow{2}{*}{26M} & \multirow{2}{*}{21M} \\
                                    & \textbf{MP} & \textbf{0.655*±0.01} & \textbf{0.568±0.01} & \textbf{0.991±0.003} &
                                    \textbf{0.35±0.00}
                                    \\
        \hline
        \multirow{1}{*}{12} & SP & 0.637±0.01 & 0.567±0.02 & 2.980±0.008 & -- & 90M & -- \\
                            %& & & & & \\
        \hline
    \end{tabular}
\end{table*}



==> tables/two_tables.tex <==
\begin{table*}[h]
\caption{Wav2Vec 2.0 results and training time. We report the number of transformer layers trained (`Layers'), activation and valence CCC on MSP-Podcast ``Test1" split (`Act' and `Val'), wall-clock training time in hours for 5 epochs (`Time'), and number of trainable parameters ('Params'). We report results for single precision (SP) and mixed precision (MP) separately. * indicates statistically significant improvement, and $\dagger$ indicates statistically significant decrease from full 12-layer finetune. Caching results are reported relative to their partial finetuning counterpart. $\uparrow$, $\downarrow$ represent increase and decrease in the value respectively. These experiments were conducted on NVIDIA A40 (non-caching) and RTX 2080 Ti (caching) GPUs.}
\label{tab:combined_results_table}
\centering
\begin{tabular}{l c c c c c||c c c c}
\hline
\multicolumn{6}{c||}{\textbf{Non-Caching Results}} & \multicolumn{4}{c}{\textbf{Relative Caching Results}} \\

\textbf{Layers} & \textbf{Precision} & \textbf{Act} & \textbf{Val} & \textbf{Time (h)} & \textbf{Params} & \textbf{Act} & \textbf{Val} & \textbf{Time (h)} & \textbf{Params} \\

% \textbf{Layers} & \textbf{Precision} & \textbf{Act} & \textbf{Val} & \textbf{Time (h)} & \textbf{Params} \\
% &&&&&&\textbf{Act}&\textbf{Val}&\textbf{Time (h)}&\textbf{Params}\\
\hline
\multirow{1}{*}{LoRA} & SP & 0.623±0.02 & 0.506$\dagger$±0.01 & 2.476±0.02 & 300K & -- & -- & -- & -- \\
\hline
\multirow{2}{*}{1} & SP & 0.622±0.02 & 0.458$\dagger$±0.01 & 2.443±0.002 & \multirow{2}{*}{12M} & .015$\uparrow$ & .049$\uparrow$ & 1.75$\downarrow$ & \multirow{2}{*}{7M}\\
& MP & 0.625±0.01 & 0.462$\dagger$±0.01 & 0.965±0.01&& .009$\uparrow$ & .046$\uparrow$ & 0.71$\downarrow$ & \\
\hline
\multirow{2}{*}{2} & SP & 0.638±0.01 & 0.508$\dagger$±0.01 & 2.477±0.01 & \multirow{2}{*}{19M}& .001$\downarrow$ & .001$\downarrow$ & 1.79$\downarrow$& \multirow{2}{*}{14M} \\
& MP & 0.645±0.01 & 0.507$\dagger$±0.004 & 0.982±0.003 && .011$\downarrow$ & .001$\uparrow$ & 0.73$\downarrow$ & \\
\hline
\multirow{2}{*}{\textbf{3}} & SP & 0.648±0.01 & 0.565±0.002 & 2.519±0.02 & \multirow{2}{*}{26M} & .004$\downarrow$ & .007$\downarrow$* & 1.50$\downarrow$ & \multirow{2}{*}{21M}\\
& \textbf{MP} & \textbf{0.655*±0.01} & \textbf{0.568±0.01} & 0.991±0.003 && .016$\downarrow$* & .013$\downarrow$ & 0.64$\downarrow$ & 
\\
\hline
\multirow{2}{*}{12} & SP & 0.637±0.01 & 0.567±0.02 & 2.980±0.01 & \multirow{2}{*}{90M} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--}\\
 & MP & 0.641±0.01 & 0.566±0.01 & 1.145±0.01 & & \\
%& & & & & \\
\hline
\end{tabular}
\end{table*}


